Stabilizing Quasi-Time-Optimal Nonlinear Model Predictive Control with Variable Discretization

This paper deals with the development and analysis of novel time-optimal point-to-point model predictive control concepts for nonlinear systems. Recent approaches in the literature apply a time transformation, however, which do not maintain recursive feasibility for piecewise constant control parameterization. The key idea in this paper is to introduce uniform grids with variable discretization. A shrinking-horizon grid adaptation scheme ensures convergence to a specific region around the target state and recursive feasibility. The size of the region is configurable by design parameters. This facilitates the systematic dual-mode design for quasi-time-optimal control to restore asymptotic stability and establish a smooth stabilization. Two nonlinear program formulations with different sparsity patterns are introduced to realize and implement the underlying optimal control problem. For a class of numerical integration schemes, even nominal asymptotic stability and true time-optimality are achieved without dual-mode. A comparative analysis as well as experimental results demonstrate the effectiveness of the proposed techniques.

==> tikzexternalize.tex <==
% !TeX encoding = UTF-8

% Externalize tikz image
% Many tikz images or tikz images with lots of data can imply a full latex buffer and therefore stop the comilation.
% If you enable externalization, tikz images are precompiled into an eps/pdf image.
% They are recompiled automatically after updating the tikz image (make sure to use recent Latex Distributions (2014+)) 
% All you need to do is to add an argument (enable-write18 or shell-escape) to the latex executable 
% in order to allow system calls:
% On Windows systems:
% 	 latex.exe [other arguments] -enable-write18 %.tex
% 	 pdflatex.exe [other arguments] -enable-write18 %.tex
% On Unix systems (Mac/Linux):
% 	 latex.exe [other arguments] -shell-escape %.tex
% 	 pdflatex.exe [other arguments] -shell-escape %.tex

\ifnum\pdfshellescape=1
% System calls enabled
%\usetikzlibrary{external} % not up to date at the moment
\usepgfplotslibrary{external}


%\ifpdf
%%%%%   DEPRECATED. Update pgfplots package (>Sept 2014). 
%%%%%				The new version automatically distinguishes between pdflatex and dvips.
%%%%%				Uncomment only if you still have problems.
%%%%%				This code will be removed in further versions.
%\else  % only for latex dvi/ps
%	\tikzset{external/system call={latex \tikzexternalcheckshellescape -halt-on-error
%	-interaction=batchmode -jobname "\image" "\texsource" && % replace && with ; in TexLive u.a.
%	dvips -o "\image".ps "\image".dvi  % && ps2eps "\image.ps"
%	}}
%\fi

\tikzexternalize[prefix=images/tikz-extern/, % folder to store precompiled tikz images (Make sure, folder already exists!!!)
optimize command away=\includepdf ] % avoid conflicts with the pdfpages packages 

% Some packages are not compatible with externalization. Create wrapped code to disable externalization:
\makeatletter
\AtBeginDocument{
	% for those using the todonodes package: this command disables the externalization mechanism from the inserted todonotes.
	\@ifpackageloaded{todonotes}{ 
		\renewcommand{\todo}[2][]{\tikzexternaldisable\@todo[#1]{#2}\tikzexternalenable} 
	}{}
	% missing-?gure package:
	\@ifpackageloaded{xmissingfigure}{ 
		\newcommand{\xmissingfigure}[2][]{\tikzexternaldisable\missingfigure[#1]{#2}\tikzexternalenable}
	}{}
}
\makeatother
\fi


% if you are using older latex distributions (<2014), the precompiled tikz images are not updated automatically, therefore run this command to update all images:
%\tikzset{external/force remake} % Recompile all tikz images

% Some helpful commands
\newcommand{\externalizeNext}{\tikzset{external/force remake=true}} % Force externalizing the next tikz picture (but tikzexternalize must be enabeld at all)
\newcommand{\externalizeOn}{\tikzset{external/export=true}} % Enable tikz externalizing for all figure splaced afterwards
\newcommand{\externalizeOff}{\tikzset{external/export=false}} % Disable tikz exernalizing for all figures placed afterwards

% fix compatibility problems with defernumbers of biblatex
\ifnum\pdfshellescape=1
\tikzifexternalizing{
	\ExecuteBibliographyOptions{defernumbers=false}
}{}
\fi

